Controlling Data Access Load in Distributed Systems

Distributed systems store data objects redundantly to balance the data access load over multiple nodes. Load balancing performance depends mainly on 1) the level of storage redundancy and 2) the assignment of data objects to storage nodes. We analyze the performance implications of these design choices by considering four practical storage schemes that we refer to as clustering, cyclic, block and random design. We formulate the problem of load balancing as maintaining the load on any node below a given threshold. Regarding the level of redundancy, we find that the desired load balance can be achieved in a system of $n$ nodes only if the replication factor $d = \Omega(\log(n)^{1/3})$, which is a necessary condition for any storage design. For clustering and cyclic designs, $d = \Omega(\log(n))$ is necessary and sufficient. For block and random designs, $d = \Omega(\log(n))$ is sufficient but unnecessary. Whether $d = \Omega(\log(n)^{1/3})$ is sufficient remains open. The assignment of objects to nodes essentially determines which objects share the access capacity on each node. We refer to the number of nodes jointly shared by a set of objects as the \emph{overlap} between those objects. We find that many consistently slight overlaps between the objects (block, random) are better than few but occasionally significant overlaps (clustering, cyclic). However, when the demand is ''skewed beyond a level'' the impact of overlaps becomes the opposite. We derive our results by connecting the load-balancing problem to mathematical constructs that have been used to study other problems. For a class of storage designs containing the clustering and cyclic design, we express load balance in terms of the maximum of moving sums of i.i.d. random variables, which is known as the scan statistic. For random design, we express load balance by using the occupancy metric for random allocation with complexes.

==> proofs/lm_P_m_lambda_nondecreasing_in_b.tex <==
The proof consists of two steps. First, we show that $\mathcal{P}^{(b)}_{b \cdot m, \lambda/b}$ is monotonic in $b$. Then, we show that $\mathcal{P}^{(b)}_{b \cdot m, \lambda/b}$ is non-decreasing in $b$.

Let $M^{(x)}$ be the maximum number of balls in any bin when $x$ balls are thrown into $n$ bins with replacement. Then, following the discussion in Sec.~\ref{sec:1_choice}, we can express the probability of robust data access for single-choice allocations with $b > 1$ objects per node as
\begin{equation}
    \mathcal{P}^{(b)}_{b \cdot m, \lambda/m} = \Prob{M^{(bm)} \leq b\mu},
\label{eq:P_bm_lambda_over_m_in_Pr_bm_leq_bmu}
\end{equation}
where $\mu = \lfloor{1/\lambda}\rfloor$.

\vspace{1ex}
\noindent
\textbf{Step 1: $\Prob{M^{(bm)} \leq b\mu}$ is monotonic}:\space 
Using the generalized scheme of allocation as described in \cite[Chapter II]{RandomAllocations:KolchinSC78}, we can express $\Prob{M^{(bm)} \leq b\mu}$ as
\[
    \Prob{M^{(bm)} \leq b\mu} = \Prob{\xi_1 \leq b\mu, \dots, \xi_n \leq b\mu ~\mid~ \xi_1 + \dots + \xi_n = bm}
\]
where $\xi_i$ are i.i.d. Poisson with mean value $bm/n$. We can rewrite this expression as
\begin{equation}
    \Prob{M^{(bm)} \leq b\mu} = \Prob{y_1 \leq \mu, \dots, y_n \leq \mu ~\mid~ y_1 + \dots + y_n = m}
\label{eq:Pr_M_bm_leq_bmu_in_yi}
\end{equation}
where $y_i$ are i.i.d. random variables given by $\xi_i/b$.
Notice that, as $b$ increases, the expression for $\Prob{M^{(bm)} \leq b\mu}$ stays the same except the distribution of $y_i$.
As $b$ increases, the mean value of $y_i$ stays fixed at $m/n$ while its variance decreases as $1/b$. In other words, as $b$ increases, $y_i$ stays as scaled Poisson random variables with a fixed mean but reduced variance.

By the properties of Poisson distribution, we know that $\Prob{y_i \leq \mu}$ is non-decreasing in $b$.
Therefore, if we assume that $\Prob{M^{(bm)} \leq b\mu}$ is non-decreasing as we increment $b$ from $1$ to $2$, then we can conclude that it will also be non-decreasing as we increment $b$ from any $i > 1$ to $i + 1$. Similarly, if we assume the opposite, i.e., $\Prob{M^{(bm)} \leq b\mu}$ is non-increasing as we increment $b$ from $1$ to $2$, then we can conclude that it will also be non-increasing as we increment $b$ from any $i > 1$ to $i + 1$.

\vspace{1ex}
\noindent
\textbf{Step 2: $\Prob{M^{(bm)} \leq b\mu}$ is non-decreasing}:\space 
Recall that $y_i$ is a scaled Poisson with fixed mean value at $m/n$ and variance going down as $1/b$. In the limit $b \to \infty$, the distribution of $y_i$ will concentrate on its mean. Hence $y_i$ will be a constant with value $m/n$. Inspecting \eqref{eq:Pr_M_bm_leq_bmu_in_yi} with this information, we find that $\Prob{M^{(bm)} \leq b\mu} = 1$ for $\mu \geq m/n$ in the limit $b \to \infty$.

In the first step, we established that $\Prob{M^{(bm)} \leq b\mu}$ is a monotonic sequence in $b$. We found that the sequence converges to $1$ as $b \to \infty$. These, together with the fact that $\Prob{M^{(bm)} \leq b\mu}$ is a cumulative distribution function, it has to be non-decreasing in $b$.

Overall, putting step 1 and 2 together and \eqref{eq:P_bm_lambda_over_m_in_Pr_bm_leq_bmu}, we show that $\mathcal{P}^{(b)}_{b \cdot m, \lambda/b}$ is non-decreasing in $b$.

% We can implement the $2m$-balls-into-$n$-bins process by executing two i.i.d. $m$-balls-into-$n$-bins processes, and then taking their superposition. We refer to the two sequences of bins, which are generated by the two i.i.d. $m$-balls-into-$n$-bins processes, as \emph{bin-sequence-$1$} and \emph{bin-sequence-$2$}, and refer to their superposition as the \emph{super-bin-sequence}. For instance, suppose $n=3$ and $m=3$. Let the number of balls in bin-sequence-$1$ and -$2$ be given as $[2, 1, 0]$ and $[1, 1, 1]$. Their the super-bin-sequence would be given as $[3, 2, 1]$.
% maximum load $M^{(2m)}$ in the original $2m$-balls-into-$n$-bins process is given by the maximum load in the super-bin-sequence. We denote the maximum load in bin-sequence-$1$ and -$2$ as $M_1^{(m)}$ and $M_2^{(m)}$ respectively. Given that bin-sequence-$1$ and -$2$ are generated by independent and identical processes, $M_1^{(m)}$ and $M_2^{(m)}$ are i.i.d. as $M^{(m)}$.

% By the law of total probability, we have
% \begin{equation}
% \begin{split}
%   \Prob{M^{(2m)} \leq 2\mu} &= \Prob{M^{(2m)} \leq 2\mu \;\bigl|\;  M^{(m)} > \mu} \Prob{M^{(m)} > \mu} \\
%   &+ \Prob{M^{(2m)} \leq 2\mu \;\bigl|\;  M^{(m)} \leq \mu} \Prob{M^{(m)} \leq \mu}.
% \end{split}
% \label{eq:Pr_M_2m_leq_2mu}
% \end{equation}

% Let us now assume that 
% \begin{equation}
%     \Prob{M^{(m)} \leq \mu} \leq \Prob{M^{(2m)} \leq 2\mu}.
% \label{eq:assume_Pr_M_m_leq_mu__leq__Pr_M_2m_leq_2mu}
% \end{equation}
% This together with $\eqref{eq:Pr_M_2m_leq_2mu}$ implies that 

% \eqref{eq:assume_Pr_M_m_leq_mu__leq__Pr_M_2m_leq_2mu}

==> proofs/lm_P_m_lambda_nondecreasing_in_b_deprecated.tex <==
We write the proof in two steps for readability. First, we show that the inequality given in \eqref{eq:Pr_m_lambda_decays_in_b} holds for $b = 2$. Then we generalize it for any $b > 1$.

\vspace{1ex}
\noindent
\textbf{When $b = 2$}:\space 
Here we relate the systems with $b=1$ and $b=2$ to each other for a given number of storage nodes $n$. Let $M^{(m)}$ (resp. $M^{(2m)}$) be the maximum number of balls in any bin when $m$ (resp. $2m$) balls are thrown into $n$ bins with replacement. Then, following the discussion in Sec.~\ref{sec:1_choice}, we can express the probability of robust data access for systems with $b=1$ and $b=2$ as follows
\[
    1 - \mathcal{P}^{(1)}_{m, \lambda} = \Prob{M^{(m)} > \mu}, 
    \quad 
    1 - \mathcal{P}^{(2)}_{2m, \lambda/2} = \Prob{M^{(2m)} > 2\mu},
\]
where $\mu = \lfloor{1/\lambda}\rfloor$.
We can implement the $2m$-balls-into-$n$-bins process by executing two i.i.d. $m$-balls-into-$n$-bins processes, and then taking their superposition. We refer to the two sequences of bins, which are generated by the two i.i.d. processes of $m$-balls-into-$n$-bins, as \emph{bin-sequence-$1$} and \emph{bin-sequence-$2$}, and refer to their superposition as the \emph{super-bin-sequence}. For instance, suppose $n=3$ and $m=3$. Let the number of balls in bin-sequence-$1$ and -$2$ be given as $[2, 1, 0]$ and $[1, 1, 1]$. Their the super-bin-sequence would be given as $[3, 2, 1]$.
Maximal load $M^{(2m)}$ in the original $2m$-balls-into-$n$-bins process is given by the maximal load in the super-bin-sequence. We denote the maximal load in bin-sequence-$1$ and -$2$ as $M_1^{(m)}$ and $M_2^{(m)}$ respectively. For the maximal load $M^{(2m)}$ in the super-bin-sequence to be larger than $2\mu$, it is necessary to have $M_1^{(m)} > \mu$ or $M_2^{(m)} > \mu$. Otherwise, the superposition of \emph{any} two bins in bin-sequence-$1$ and -$2$ would not yield $M^{(2m)} > 2\mu$. This necessary condition gives us the following inequality
\begin{equation}
    \Prob{M^{(2m)} > 2\mu}
    \leq \Prob{M_1^{(m)} > \mu ~~\textrm{or}~~ M_2^{(m)} > \mu}
\label{eq:upper_bound_on_Pr_M_2m_gt_2mu}
\end{equation}
where the right hand side is equal to
\[ 
    \Prob{M_1^{(m)} > \mu} + \Prob{M_2^{(m)} > \mu} - \Prob{M_1^{(m)} > \mu, M_2^{(m)} > \mu}. 
\]
Given that bin-sequence-$1$ and -$2$ are i.i.d. processes, the random variables $M_1^{(m)}$ and $M_2^{(m)}$ are also i.i.d. as $M^{(m)}$. Therefore, we can write the above expression as
\[
    2\Prob{M^{(m)} > \mu} - \Prob{M^{(m)} > \mu}^2.
\]
Substituting this in the right hand side of \eqref{{eq:upper_bound_on_Pr_M_2m_gt_2mu}}, we obtain    
\[
    \Prob{M^{(2m)} > 2\mu} 
    \leq 2\Prob{M^{(m)} > \mu} - \Prob{M^{(m)} > \mu}^2.
\]
Replacing the left and right hand sides of the inequality above and adding $1$ in both sides gives us
\[
    \left(1 - \Prob{M^{(m)} > \mu}\right)^2 \leq 1 - \Prob{M^{(2m)} > 2\mu},
\]
which can also be written as
\[
    \Prob{M^{(m)} \leq \mu}^2 \leq \Prob{M^{(2m)} \leq 2\mu}.
\]
Taking square root of each side we have
\begin{equation}
    \Prob{M^{(m)} \leq \mu} \leq \Prob{M^{(2m)} \leq 2\mu}^{1/2}.
\label{eq:Pr_M_m_leq_mu__leq__sqrt_Pr_M_2m_leq_2mu}
\end{equation}
By the discussion in Sec.~\ref{sec:1_choice}, we can write the above inequality as
\begin{equation*}
    \mathcal{P}^{(1)}_{m, \lambda} \leq \left(\mathcal{P}^{(b)}_{2m, \lambda/2}\right)^{1/2},
% \label{eq:Pr_P_m_lambda__leq__sqrt_P_2m_lambda_over_2}
\end{equation*}
which proves \eqref{eq:Pr_m_lambda_decays_in_b} for $b=2$.

\vspace{1ex}
\noindent
\textbf{Generalization for any $b > 1$}:\space 
Here we extend the discussion given above for $b=2$ to any $b > 1$.
Let $M^{(m)}$ (resp. $M^{(b \cdot m)}$) be the maximum number of balls in any bin when $m$ (resp. $b \cdot m$) balls are thrown into $n$ bins with replacement. Then, we can express the probability of robust data access for systems with $b=1$ and $b$ as follows
\[
    1 - \mathcal{P}^{(1)}_{m, \lambda} = \Prob{M^{(m)} > \mu}, 
    \quad 
    1 - \mathcal{P}^{(b)}_{b \cdot m, \lambda/b} = \Prob{M^{(b \cdot m)} > b\mu},
\]
where $\mu = \lfloor{1/\lambda}\rfloor$.
We can implement the $b \cdot m$-balls-into-$n$-bins process by executing $b$ i.i.d. $m$-balls-into-$n$-bins processes, and then taking their superposition. We refer to the sequences of bins, which are generated by the $b$ i.i.d. processes of $m$-balls-into-$n$-bins, as \emph{bin-sequence-$i$} for $i = 1, \ldots, b$, and refer to their superposition as the \emph{super-bin-sequence}.
Maximal load $M^{(b \cdot m)}$ in the original $b \cdot m$-balls-into-$n$-bins process is given by the maximal load in the super-bin-sequence. We denote the maximal load in bin-sequence-$i$ as $M_i^{(m)}$. For the maximal load $M^{(b \cdot m)}$ in the super-bin-sequence to be larger than $b\mu$, it is necessary to have $M_i^{(m)} > \mu$ hold for at least one $i$. Otherwise, the superposition of \emph{any} $b$ bins across all bin-sequence-$i$ would not yield $M^{(b \cdot m)} > b\mu$. This necessary condition gives us the following inequality
\begin{equation}
    \Prob{M^{(b \cdot m)} > b\mu}
    \leq \Prob{\bigcup_{i=1}^{b} \{M_i^{(m)} > \mu\}}
\label{eq:upper_bound_on_Pr_M_bm_gt_bmu}
\end{equation}
where the right-hand side is equal to
\[ 
    \sum_{i=1}^m (-1)^{i+1} \left(\sum_{1 \leq j_1 < \ldots < j_i \leq m} \Prob{M_{j_1}^{(m)} > \mu, \ldots, M_{j_i}^{(m)} > \mu} \right). 
\]
Given that bin-sequence-$i$ are i.i.d. processes, the random variables $M_i^{(m)}$ are also i.i.d. as $M^{(m)}$. Therefore, we can write the above expression as
\[ 
    \mathbf{\Epsilon} = \sum_{i=1}^m (-1)^{i+1} \left(\sum_{1 \leq j_1 < \ldots < j_i \leq m} \Prob{M_{j_1}^{(m)} > \mu} \cdot \ldots \cdot \Prob{M_{j_i}^{(m)} > \mu} \right).
\]
Substituting $\mathbf{\Epsilon}$ in the right hand side of \eqref{{eq:upper_bound_on_Pr_M_bm_gt_bmu}}, we obtain    
\[
    \Prob{M^{(b \cdot m)} > b\mu} \leq \mathbf{\Epsilon}.
\]
Replacing the left and right hand sides of the inequality above and adding $1$ in both sides gives us
\[
    \left(1 - \Prob{M^{(m)} > \mu}\right)^b \geq 1 - \Prob{M^{(b \cdot m)} > b\mu},
\]
which can also be written as
\[
    \Prob{M^{(m)} \leq \mu}^b \geq \Prob{M^{(b \cdot m)} \leq b\mu}.
\]
Taking $1/b$ to the power of each side, we have
\begin{equation}
    \Prob{M^{(m)} \leq \mu} \leq \Prob{M^{(b \cdot m)} \leq b\mu}^{1/b}.
\label{eq:Pr_M_m_leq_mu__leq__Pr_M_bm_leq_bmu_pow_1_over_b}
\end{equation}

By the discussion in Sec.~\ref{sec:1_choice}, we can write the above inequality as
\begin{equation*}
    \mathcal{P}^{(1)}_{m, \lambda} \leq \left(\mathcal{P}^{(b)}_{b \cdot m, \lambda/b}\right)^{1/b},
% \label{eq:Pr_P_m_lambda__leq__P_M_bm_lambda_over_b_pow_1_over_b}
\end{equation*}
which proves \eqref{eq:Pr_m_lambda_decays_in_b} for any $b > 1$.

% #####################################  Part 2  ###################################### %
% \begin{lemma}
% Let $\mathcal{P}^{(b)}_{b \cdot m, \lambda/b}$ be the probability of robust data access (as defined in Def.~\ref{def:P_m_lambda}) for a system where (1) each node stores $b > 1$ different objects with no redundancy, (2) proportion of active objects stays the same as $m/n$ with increasing $b$, (3) cumulative demand stays the same as $m\lambda$ with increasing $b$. Then, $\mathcal{P}^{(b)}_{b \cdot m, \lambda/b}$ is non-decreasing in $b$ if $m/(n\ln(n)) \leq x$ in the limit as $m, n \to \infty$ where $x$ is a positive constant.
% \label{lm:Pr_m_lambda_nondecreasing_in_b}
% \end{lemma}
% \begin{proof}
%   See Appendix~\ref{subsec:proof_lm_Pr_m_lambda_nondecreasing_in_b}.
% \end{proof}

% \vspace{1ex}
% \noindent
% \textbf{As $b$ goes from $1$ to $2$}:\space 
% We first relate the systems with $b=1$ and $b=2$ to each other for a given number of storage nodes $n$. Let $M^{(m)}$ (resp. $M^{(2m)}$) be the maximum number of balls in any bin when $m$ (resp. $2m$) balls are thrown into $n$ bins with replacement. Then, following the discussion in Sec.~\ref{sec:1_choice}, we can express the probability of robust data access for systems with $b=1$ and $b=2$ as follows
% \[
%     \mathcal{P}^{(1)}_{m, \lambda} = \Prob{M^{(m)} \leq \mu}, 
%     \quad 
%     \mathcal{P}^{(2)}_{2m, \lambda/2} = \Prob{M^{(2m)} \leq 2\mu},
% \]
% where $\mu = \lfloor{1/\lambda}\rfloor$.

% We can implement the $2m$-balls-into-$n$-bins process by executing two i.i.d. $m$-balls-into-$n$-bins processes, and then taking their superposition. We refer to the two sequences of bins, which are generated by the two i.i.d. $m$-balls-into-$n$-bins processes, as \emph{bin-sequence-$1$} and \emph{bin-sequence-$2$}, and refer to their superposition as the \emph{super-bin-sequence}. For instance, suppose $n=3$ and $m=3$. Let the number of balls in bin-sequence-$1$ and -$2$ be given as $[2, 1, 0]$ and $[1, 1, 1]$. Their the super-bin-sequence would be given as $[3, 2, 1]$.
% maximum load $M^{(2m)}$ in the original $2m$-balls-into-$n$-bins process is given by the maximum load in the super-bin-sequence. We denote the maximum load in bin-sequence-$1$ and -$2$ as $M_1^{(m)}$ and $M_2^{(m)}$ respectively. Given that bin-sequence-$1$ and -$2$ are generated by independent and identical processes, $M_1^{(m)}$ and $M_2^{(m)}$ are i.i.d. as $M^{(m)}$.

% By the law of total probability, we have
% \begin{equation}
%   \begin{split}
%       \Pr\left\{M^{(2m)} > 2\mu\right\} &= \Pr\left\{M^{(2m)} > 2\mu \;\bigl|\;  M^{(m)} > \mu\right\} \Pr\left\{M^{(m)} > \mu\right\} \\
%       &+ \Pr\left\{M^{(2m)} > 2\mu \;\bigl|\;  M^{(m)} \leq \mu\right\} \Pr\left\{M^{(m)} \leq \mu\right\}.
%   \end{split}
%   \label{eq:Pr_M_2m_leq_2mu}
%   \end{equation}
% We use the split process described above to find bounds on $\Pr\left\{M^{(2m)} > 2\mu \;\bigl|\;  M^{(m)} > \mu\right\}$ and $\Pr\left\{M^{(2m)} > 2\mu \;\bigl|\;  M^{(m)} \leq \mu\right\}$, substituting which then will give us the bound on $\Pr\left\{M^{(2m)} > 2\mu\right\}$.

% We first derive the bound on $\Pr\left\{M^{(2m)} > 2\mu \;\bigl|\; M^{(m)} \leq \mu\right\}$ in \eqref{eq:Pr_M_2m_leq_2mu}. Suppose that the maximum load $M_1^{(m)}$ in bin-sequence-$1$ is $\leq \mu$. This implies that the number of balls in any bin is $\leq \mu$. It is then necessary for the maximum load $M_2^{(m)}$ in bin-sequence-$2$ to be $\geq \mu$ in order for the maximum load in the super-bin-sequence to be $2\mu$. In other words, $M_2^{(m)} > \mu$ is a necessary condition for $M^{(2m)} > 2\mu$ given that $M_1^{(m)} \leq \mu$. Given also that $M_1^{(m)}$ and $M_2^{(m)}$ are i.i.d. as $M^{(m)}$, we have
% \begin{equation}
%     \Pr\left\{M^{(2m)} > 2\mu \;\bigl|\; M^{(m)} \leq \mu\right\} \leq \Pr\left\{M^{(m)} \leq \mu\right\}.
% \label{eq:upper_bound_on_Pr_M_2m_gt_2mu_given_M_m_leq_mu}
% \end{equation}
% We next derive the bound on $\Pr\left\{M^{(2m)} > 2\mu \;\bigl|\; M^{(m)} > \mu\right\}$ in \eqref{eq:Pr_M_2m_leq_2mu}. We will refer to the node with maximum load in bin-sequence-$1$ and -$1$ as node-max-$1$ and -$2$. Given $M_1^{(m)} > \mu$, there are three cases in which $M_2^{(m)} > \mu$: (1) Two nodes node-max-$1$ and -$2$ are superposed on the same node in super-bin-sequence. We refer to this event as $\{\text{node-max-$1$ and -$2$ superposed}\}$. 

% For the maximum load $M^{(2m)}$ in the super-bin-sequence to be larger than $2\mu$, it is necessary to have $M_1^{(m)} > \mu$ or $M_2^{(m)} > \mu$. Otherwise, the superposition of \emph{any} two bins in bin-sequence-$1$ and -$2$ would not yield $M^{(2m)} > 2\mu$.

% \vspace{1ex}
% \noindent
% \textbf{As $b$ goes from $2$ to $3$}:\space 



==> proofs/lm_limiting_P_m_lambda_nondecreasing_in_b.tex <==
Let $M^{(b \cdot m)}$ be the maximum number of balls in any bin when $b \cdot m$ balls are thrown into $n$ bins. Then, following the discussion in Sec.~\ref{sec:1_choice}, we can express the probability of robust data access as follows
\[
    \mathcal{P}^{(b)}_{b \cdot m, \lambda/b} = \Prob{M^{(b \cdot m)} \leq b\mu},
\]
where $\mu = \lfloor{1/\lambda}\rfloor$.

The remainder of the proof consists of two steps.

\vspace{1ex}
\noindent
\textbf{If $bm/(n\ln(n)) \to x$ as $m, n \to \infty$}:\space 
In this case, by  \cite[Theorem 2]{RandomAllocations:KolchinSC78},  we know that
\[
    \Prob{M^{(bm)} \leq b\mu} \to \Exp{-\frac{\lambda \gamma^{b\mu - r + 1}}{1 - \gamma}},
\]
where $\gamma$ is the root of the equation $\gamma + x(\ln(\gamma) - \gamma + 1) = 0$ in an interval $0 < \gamma < 1$, and $r$ is chosen such that
\[
    n \frac{(bm/n)^r}{r!} \Exp{-bm/n} \to \lambda.
\]
As $b$ increases, $x$ increases, $\gamma$ decreses. $r$ should also increase 


\vspace{1ex}
\noindent
\textbf{If $m/(n\ln(n)) \to 0$ as $m, n \to \infty$}:\space 

if $m/(n\ln(n)) \leq x$ in the limit as $m, n \to \infty$ where $x$ is a positive constant

==> proofs/thm_P_bounds_for_random.tex <==
Suppose that the number of active objects $A$ is given. 
Given that the demand of active objects is equal to $\lambda$, cumulative demand for the active objects is given as $A \cdot \lambda$.
Given that the service choices for each object are selected independently and randomly, the span of $A$ active objects is equal to the occupancy of random allocations with $d$-size complexes, $N_{n, d, A}$. This, together with the maximal load requirement, we can express the cumulative capacity available for the active objects as $m \cdot N_{n, d, A}$.

As discussed in Sec.~\ref{subsec:calculating_P_for_given_storage_allocation}, considering only a subset of the demand-capacity conditions given in \eqref{eq:modified_cap_region_w_service_choice_spans} gives us an upper bound on $\mathcal{P}$. 
So considering the condition for only $A$ active objects at a time gives us an upper bound, which is stated as
\[
    \Prob{N_{n, d, A} \geq A \cdot \lambda / m}.
\]
As the expression above is an upper bound, its expectation with respect to $A$ is also an upper bound. This gives us \eqref{eq:P_upper_bound_for_random}.

==> proofs/thm_P_lower_bound_for_clustering_w_bounded_demand.tex <==
Recall from the proof of Lemma~\ref{lm:P_clustering}, the probability that a single cluster meets the maximal load requirement is given by
\[
    \mathcal{P}_c = \Prob{\rho_1 + \ldots + \rho_d \leq m \cdot d}.
\]
Let us denote the sample average demand as $\bar{\rho} = (\rho_1 + \ldots + \rho_d) / d$.
Then we can write $\mathcal{P}_c$ as
\begin{equation}
    \mathcal{P}_c = \Prob{\bar{\rho} \leq m}.
\label{eq:P_c_w_sample_average}
\end{equation}
Let us now use $\mu$ to denote the average object demand $\E{\Lambda}$, and use $\mathcal{Q}_c$ to denote $1 - \mathcal{P}_c$.
By subtracting $\mu$ from both sides of the inequality in \eqref{eq:P_c_w_sample_average}, we can express $\mathcal{Q}_c$ as
\[
    \mathcal{Q}_c = \Prob{\bar{\rho} > m - \mu}.
\]
Given this expression and the fact that the demand distribution is bounded as $a \leq \Lambda \leq b$, we can use Hoeffding's inequality to bound $\mathcal{Q}_c$ from above as
\[
    \mathcal{Q}_c = \Prob{\bar{\rho} > m - \mu} \leq \exp{-d \cdot 2(m - \mu)^2 / (b - a)^2}.
\]
This gives the following lower bound on $\mathcal{P}_c$
\[
    \mathcal{P}_c \geq 1 - \exp{-d \cdot 2(m - \mu)^2 / (b - a)^2}.
\]
Substituting this lower bound in \eqref{eq:P_clustering} gives us \eqref{eq:P_lower_bound_for_clustering_w_bounded_demand}.

